ResidualSketch: Enhancing Layer Efficiency and Error Reduction in Hierarchical Heavy Hitter Detection with ResNet Innovations

In network management, swiftly and accurately identifying traffic anomalies, including Distributed Denial-of-Service (DDoS) attacks and unexpected network disruptions, is essential for network stability and security. Key to this process is the detection of Hierarchical Heavy Hitters (HHH), which significantly aids in the management of high-speed IP traffic. This study introduces ResidualSketch, a novel algorithm for HHH detection in hierarchical traffic analysis. ResidualSketch distinguishes itself by incorporating Residual Blocks and Residual Connections at crucial layers within the IP hierarchy, thus mitigating the Gradual Error Diffusion (GED) phenomenon in previous methods and reducing memory overhead while maintaining low update latency. Through comprehensive experiments on various datasets, we demonstrate that ResidualSketch outperforms existing state-of-the-art solutions in terms of accuracy and update speed across multiple layers of the network hierarchy. All related codes of ResidualSketch are open-source at GitHub.

==> TongYang/intro.tex <==
%!TEX root = timingSGI.tex

\presec
\section{Introduction}\label{sec:introduction}
\postsec
%\vspace{-0.05in}
\label{sec:algorithm}
\presub
\subsection{Background and Motivations}
\postsub


Data stream processing is a significant issue arising in many applications, like intrusion detection systems \cite{Oh2006Anomaly,Faisal2012Securing}, financial data trackers \cite{Ball2014A,Gyurk2013Extracting}, sensor networks \cite{Hu2012Stability, Figueiredo2007Data}, \etc\  
%
A data stream is composed of an unbounded sequence of items arriving at high speed. 
%
Contrary to traditional static datasets, data streams require to be processed in real time, \ie, in one pass, and in $O(1)$ update time. 
%
Due to the large volume and high speed, it is difficult and often unnecessary to store the whole data streams completely.
%
Moreover, large-scale data stream processing applications are usually distributed. Information exchange is needed among multiple hosts which observe local streams. Transporting complete data streams requires a lot of bandwidth and is far from communication efficient.
%
Instead, one effective choice is to maintain a small summary of the data stream.
%Fortunately, it is usually not necessary to return an accurate result in data stream queries.
%Therefore, probabilistic data structures are usually applied.
%

Sketches, a kind of probabilistic data structures, achieving memory efficiency at the cost of introducing small errors, have been widely used as the summary of data streams.
%They summarize the data stream with small and controllable errors. We call these data structures sketches for the data stream.
Sketches only need small memory usage, which makes it possible to store them in fast memory, such as L2 caches in CPU and GPU chips, and Block RAM in FPGA \cite{FPGADatasheet}.
%
Typical sketches include the Bloom filter \cite{BF1970}, the CM sketch \cite{cmsketch}, the CU sketch \cite{cusketch}, \etc \ 
%
However, these sketches cannot delete the out-dated items.
%


In applications of data streams, people usually focus on the most recent items, which reflect the current situation and the future trend.
%
For example, in financial analysis, people focus on the current finance trend, and in intrusion detection systems, people are mainly concerned about the recent intrusions.
%
Therefore, it is usually necessary to downgrade the significance of old items and discard them when appropriate.
Otherwise, they will bring a waste of memory, and also introduce noise to the analysis of recent items.
%
It is an important issue to develop probabilistic data structures which can automatically ``forget'' old items and focus on recent items.

%There have been several time-decay query models for data streams, and among them the sliding window model \cite{..} is one of the most widely used model.
%
The most widely used model for recording recent items is the sliding window model \cite{Datar2002Maintaining}.
In this model, there is a sliding window including only the most recent items, while the items outside are forgotten (deleted).
%the window are aged and given a weight of $0$.
%
%The sliding window model can be either time-based or count-based.
%In the time-based model, only the items arriving in the last $N$ time units are included in the window.
%In the count-based model, the most recent $N$ items are included in the window.
%Whenever a new item arrives, the window moves on, adding new items and deleting out-dated items which are no longer within the sliding window.
%

There are various queries which can be implemented in the sliding window model.
%
In this paper, we focus on three kinds of fundamental queries: membership query, frequency query, and heavy hitter query.
%
Membership query is to check if an item $e$ is in the sliding window.
Frequency query is to report the frequency of an items $e$. 
Heavy hitter query is to find all the items with frequencies exceeding a threshold.


%
It is challenging to design a probabilistic data structure for the sliding window model.
%
Whenever a new item arrives, the oldest item needs to be deleted. However, it is challenging to find the oldest item, especially when the demand on memory and speed is high. 
%
We have to implement deletions in $O(1)$ time to catch up with the speed of the data stream. 
%
Moreover, we cannot store all items' ID in the sliding window, because the sliding window may be very large and it is memory-consuming to store them.

\presub
\subsection{Prior Art and Their Limitations}
\postsub
There have been quite a few algorithms on approximate queries in sliding windows. These algorithms can be divided into three kinds according to the queries they can support. 
%
The first kind supports membership queries, like the double buffering Bloom filter \cite{Chang2004Approximate}, the $A^2$ buffering Bloom filter \cite{Yoon2009Aging}, the forgetful Bloom filter \cite{Subramanyam2016Idempotent} and so on. 
%
The second kind is designed for frequency queries, like the ECM sketch \cite{papapetrou2012sketch}, the splitter windowed count-min sketch \cite{rivetti2015efficiently} and so on \cite{Chan2009Continuous,Cormode2011Tracking}. 
%
The third kind supports heavy hitter queries. This kind includes $\lambda-$sampling algorithm \cite{Hung2010Finding}, the window compact space saving (WCSS) \cite{Ran2016Heavy} and so on \cite{Lee2006A}.


%However, they have two limitations. First, these works usually
%the data stream into periods with the same length, and store $d$ most recent periods as an approximation of the sliding window. As shown in Figure \ref{gp}. When the oldest mini window is out of date, they delete it and add a new one. This is a approximation of the sliding window. The error is $\frac{1}{d}$ of the sliding window, as each mini window has to work as a unit. When only part of it overlaps with the sliding window, we still have to reckon the whole mini window in (or not). $d$ can not be very large, as it is memory consuming to store these mini windows. However, if $d$ is small, the accuracy will be poor.

However, existing algorithms have two main limitations. First, these algorithms usually need a lot of memory to achieve fine-grained deletions. When the memory space is tight, the accuracy of these algorithms is poor. 
%
Second, most existing algorithms only handles one specific query in sliding windows. 
%
However, in applications various kinds of queries are usually needed, which makes a general framework more preferred. 

\presub
\subsection{Our Proposed Solution}
\postsub

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figures/general-periods.pdf}
\precaption
\caption{Illustration of the sliding window and the Days}
\label{gp}
\end{figure}

In this paper, we propose a framework, namely \texttt{the Sliding sketch}.
%
It can be applied to most of the existing sketches and adapt them to the sliding window model.
We apply our framework to the Bloom filter \cite{BF1970}, the CM sketch \cite{cmsketch}, the CU sketch \cite{cusketch}, the Count sketch \cite{countsketch}, and the HeavyKeeper  \cite{HeavyKeeper} for experimental evaluation in Section \ref{sec:eva}.

%By varying the fundamental sketch we use, the Sliding sketch can be applied to various kinds of queries in sliding windows, like the membership query, the frequency query and the heavy hitter query.
%Next, we first give a summary of the key idea of our approach. 
%statement of the problem. Then we introduce the common model of the typical sketches. After that, we introduce how to make these sketches support deletion of out-dated information. Then we give an inspiration we get, and introduce the key technique of our framework. At last, we will give a brief analysis of why this technique works.

%1.\ppp{Problem definition:} Suppose we need to estimate the information in a sliding window which includes the most recent $N$ items.


In the following, first, we introduce the common sketch model. Second, we use a classic method to make this model support deletions of out-dated information. 
%
Third, we explain our key observation.
%
Fourth, based on the observation, we present our key technique.
%
Fifth, we explain why this technique works.
%
Finally, we give a summary of our experimental results.

\ppp{1) Sketch model:}
 A typical sketch uses $m$ buckets, which are divided into $k$ equal-sized segments. Each segment is associated with one hash function. When an item $e$ arrives, the sketch maps it into $k$ buckets using the $k$ hash functions, one in each segment, and records the information of $e$ in these buckets. We call these $k$ buckets \textbf{the $k$ mapped buckets}. 
 For queries, the sketch returns the most accurate value in the $k$ mapped buckets.

\ppp{2) Deleting out-dated information:} We split the data stream into small periods. The length of each period is $\frac{1}{d-1}$ of the sliding window. We call each period a \textbf{Day}.  In each bucket, we use $d$ fields to record the most recent $d$ periods, in order to estimate the information in the sliding window. Whenever a field is out-dated, we delete it. This method is classic and intuitive, and has been used in many prior works.

Take an example in Figure \ref{gp}.
We set $d=4$. Each Day is $\frac{1}{3}$ of the sliding window. We record the most recent $4$ Days, \ie, $Day_2 \sim Day_5$. Notice $Day_5$ is not a complete Day, and only $\delta (0\leqslant \delta<1) $ of it has passed at the query time. For convenience, we call $\delta$ the \textbf{jet lag}.

\ppp{3) Observation:} We observe that when the query time is close to the nearest \textbf{zero time}, \ie, the start time of the nearest Day, the $d$ Days we record will be very close to the sliding window. 
%
In other words, we record additional $\delta$ of the oldest Day, which is out-dated. The smaller $\delta$ is, the higher accuracy we achieve.
%
In prior works, the entire data structure works synchronously, which means all the buckets always have the same jet lag. This makes the accuracy of the data structure fluctuates according to the query time. In the worst case, the error can be $\frac{1}{d-1}$ of the sliding window plus the errors of hash collisions. Note that in the sketch model mentioned above, each item is mapped to $k$ buckets, and the most accurate value will be reported in queries. We come up with an idea: \textit{is it possible to make different buckets asynchronous and achieve that for each item there is at least one mapped bucket with a small jet lag?}.

\ppp{4) Our Key technique:} Based on the above observation, we use a scanning pointer to scan all the buckets one by one, again and again at a constant speed.
%
When the scanning pointer points to a bucket, we call this time the \textbf{zero time} of the bucket.
%
In this way, the zero time of different buckets is asynchronous.
%
At the zero time, we delete the oldest field, and insert a new field into the bucket as the unique active field. It means a new Day just started.

The above process is just like the sun and Earth.
%
The array/Earth is split into many buckets/time zones.
%
Every time when the scanning pointer/sun reaches a bucket/time zone, a new Day starts, and the out-dated information is deleted.
%
Every two buckets/time zones have different time.
%

\ppp{5) Why our framework works?} 
%
The $k$ mapped buckets of an item are separated and distributed in the $k$ equal-sized segments/\textit{continent}. It is like that the item is mapped to $k$ time zones, one in a continent. Whenever we query, there must be a continent which has just passed the zero time. The bucket in this `continent' has a small enough jet lag, to be precise, less than $\frac{2}{k}$ (proofs are provided in the technical report \cite{opensource} due to space limitation). In this way, the error is bounded to be $\frac{2}{k\times(d-1)}$ of the sliding window.
%
In contrast, existing related algorithms use the same zero time for all buckets, and thus the error can only be bounded as $\frac{1}{d-1}$ of the sliding window.

Extensive experiments and theoretical analysis show that the Sliding sketch has high accuracy with small memory usage. Experimental results show that after using our framework, the accuracy of existing sketches that do not support sliding windows becomes much higher than the algorithms for sliding windows. In membership query, the error rate of the Sliding sketch is $10\sim50$ times lower than that of the state-of-the-art sliding window algorithm. In frequency query, the ARE of the Sliding sketch is $40\sim 50$ times lower than that of the state-of-the-art sliding window algorithm. In heavy hitter query, the precision and recall of the Sliding sketch are near to $100\%$ and better than the state-of-the-art, and the ARE of the frequencies of heavy hitters in the Sliding sketch is $3 \sim 5.6$ times lower than that of the state-of-the-art sliding window algorithm.



\nop{There are two key techniques in our framework as follows.

1) The first key technique is as follows. We split the data stream into small periods and the length of each period is $\frac{1}{d-1}$ of the sliding window. We record the most recent $d$ periods to estimate the information in the sliding window.
%
We call each period a \textbf{Day}. 
Take an example in Figure \ref{gp}.
We set $d=4$. Each Day is $\frac{1}{3}$ of the sliding window. We record the most recent $4$ Days, \ie, $Day_2 \sim Day_5$. Notice $Day_5$ is not a full day, and only $\delta (0\leqslant \delta<1) $ of it has passed at the query time. For convenience, we call $\delta$ the \textbf{jet lag}.


we notice that when the query time is close to the nearest \textbf{zero time}, \ie, the start time of the nearest Day, the accuracy of this approximation will be high. 
%
In other words, the smaller $\delta$ is in Figure \ref{gp}, the higher accuracy we achieve.


%
We further notice that most of the state-of-the-art sketches map each item in the data stream into $k$ buckets, and record the information of the item by updating these buckets. 
%
In query operation, they report the most accurate value in these buckets. 
%


 We use these observations and come up with the key idea of the Sliding sketch.
 
2) The second key technique is as follows. We consider each bucket in the sketch as an time zone. Two adjacent time zone there is a constant time difference.
In this way, for each item, the $k$ hashed buckets work asynchronously, and we have proved that at least one mapped time zone/bucket has a very small jet lag $\delta$, so as to achieve high accuracy.
%


Given a typical sketch $\mathcal{S}$ composed of buckets. It is divided into $k$ equal-sized regions. Each region has $w$ buckets, and is associated with a hash function.
%
To report the information in a sliding window,
%: $N$ recent-arrival items.
%
we use $d$ small periods, or what we call \textbf{Days}, to approximate one sliding window.
%
For each Day, we record the information in one field. 
%
For any time, there is only one active Day, and we may call it \textbf{Today}. At query time $T$, we may have spent part of Today, and we use $\delta$, the jet lag, to represent this percentage. The other Days become the past. In the Sliding sketch, we store the information in Today and $d-1$ past Days.
%
Therefore, each bucket has $d$ fields, including 1 active field and $d-1$ inactive fields.
%


We use a scanning pointer to scan all the buckets one by one, again and again at constant speed.
%
Given any time, the scanning pointer points to a bucket, and we call the time the zero time of the bucket.
%
In this way, the zero time in different buckets are asynchronous.
%
At the zero time, we delete the oldest field, and insert a new field into it as the unique active field. It means a new Day has started.
%
Given a query at any time, we will get $k$ mapped buckets for the queried item. For mapped each bucket $B[i]$, jet lag $\delta$ can be computed with the distance between $B[i]$ and the scanning pointer, as the scan pointer scans at constant speed.
%
Obviously, the smaller the jet lag is, the higher accuracy $B[i]$ will achieve in this query. 
%
Fortunately, we can make sure that there is at least one bucket/time zone has the jet lag less than $\frac{2}{k\times(d-1)}$. In this way the error is bounded to be $\frac{2}{k\times(d-1)}$ of the sliding window.
%
In contrast, most existing solutions use the same zero time for all buckets, and thus the error is only bounded to be $\frac{1}{d-1}$ of the sliding window.
%
%In other words, we reduce the jet lag from 1 period to $\frac{2}{k\times(d-1)}$ period (typically, $k=10$ and $d=4$).


%storing a period close enough to the sliding window, $1 \sim 1+ \frac{2}{k\times(d-1)}$ times of it to be precisely.


%In the Sliding sketch, we also map each item $e$ into $k$ buckets. In each bucket, we split the data stream into small periods and store the information of $e$ in the last $d$ periods. In different buckets, the split points of the periods are different. By using a novel operation named \textit{clocking operation} to control the split points, we can make sure that there is at least one bucket storing a period close enough to the sliding window, $1 \sim 1+ \frac{2}{k\times(d-1)}$ times of it to be precisely. 

\ppp{6) Main experimental results:} Experiments and mathematical analysis show that the Sliding sketch have high accuracy with small memory usage. {\color{red} here is a \yt{summarization/summary??} of the experiment result}.
}

\presub
\subsection{Key contribution}
\postsub
Our key contributions are as follows:

1) We propose a generic framework named the Sliding sketch, which can be applied to most existing sketches and adapt them to sliding window models. 

2) We apply our framework to three typical kinds of queries in sliding windows: membership query (Bloom filters), frequency query (sketches of CM, CU, and Count), and heavy hitter query (HeavyKeeper). 
%
Mathematical analysis and experiments and show that the Sliding sketch achieves much higher accuracy than the state-of-the-art.

%2) We apply the Sliding sketch technique to the Bloom filter, the CM sketch, the Count sketch, the CU sketch and the heavy keeper as examples. We also implement extensive experiments to compare it with prior arts in the membership queries, the frequency queries and the heavy hitter queries. Experiments show that ....

==> TongYang/introduction.tex <==
\presec
\section{Introduction} \postsec

\subsection{Background and Motivation}
\postsub

%para 1:
Big data stream processing becomes a hot issue in recent years.
%
Many work strive to handle various tasks in data streams.
%
There are three fundamental measurement tasks: membership queries, frequency queries, and heavy hitter queries.
%
For each kind of queries, there have been a lot of solutions.
%
However, most existing solutions handle these queries in fixed time window.
%
For example, given a data stream \mathcal{S}, each item in which could appear more than once.
%
This stream is divided into many equal sized windows, each of which consists of $n$ items.
%
Given a time window with $n$ items, 1) membership queries are to check whether an input item $e$ in a specific time window; 2) frequency queries are to report how many does a input item $e$ appears in the time window.
%
Heavy hitter queries are to check whether an input item has a frequency larger than a predefined threshold.



While most of existing work focus on fixed time window queries, this paper focus on more challenging queries: queries in sliding windows.
%
In this kinds of queries, we need to answer queries of membership, frequency, and heavy hitter in the recent time window, \ie, those $w$ item recently arrived.


Queries in sliding windows are much more challenging than those in fixed window because of three reasons.
First, whenever an incoming item arrives, the information of the oldest item should be deleted from the data structure. Unfortunately, as $w$ is usually very large, it is almost impossible to know the oldest item in the sliding window.
%
Second, even if the deletion of the oldest item can be figured out, some of existing data structures do not support deletion, such as Bloom filters, CU sketches, \etc
%



\presub
\subsection{Prior Art and their limitations} \postsub

Existing solutions use different method for different kinds of queries.
For membership queries, the typical algorithms use two Bloom filters, one for active, and another for inactive, periodically exchanged.
%
For frequencies queries, ....
%
For heavy hitter queries, ...
%
In summary, all existing solutions cannot achieve high accuracy because they cannot identify the oldest item efficiently.

\presub
\subsection{Our Proposed Solution}
\postsub




\presub
\subsection{Key Contributions}
\postsub


